CONE: An Efficient COarse-to-fiNE Alignment Framework for Long Video Temporal Grounding

This paper tackles an emerging and challenging problem of long video temporal grounding~(VTG) that localizes video moments related to a natural language (NL) query. Compared with short videos, long videos are also highly demanded but less explored, which brings new challenges in higher inference computation cost and weaker multi-modal alignment. To address these challenges, we propose CONE, an efficient COarse-to-fiNE alignment framework. CONE is a plug-and-play framework on top of existing VTG models to handle long videos through a sliding window mechanism. Specifically, CONE (1) introduces a query-guided window selection strategy to speed up inference, and (2) proposes a coarse-to-fine mechanism via a novel incorporation of contrastive learning to enhance multi-modal alignment for long videos. Extensive experiments on two large-scale long VTG benchmarks consistently show both substantial performance gains (e.g., from 3.13% to 6.87% on MAD) and state-of-the-art results. Analyses also reveal higher efficiency as the query-guided window selection mechanism accelerates inference time by 2x on Ego4D-NLQ and 15x on MAD while keeping SOTA results. Codes have been released at https://github.com/houzhijian/CONE.

==> Paragraphs/1-Intro.tex <==
\section{Introduction}
Video temporal grounding~\cite{anne2017localizing,gao2017tall} aims to locate specific moments in an untrimmed video relevant to a textual user query.
This is a crucial task in multi-modal video understanding, with many practical applications such as video retrieval, video editing, and video question answering. Temporal grounding for \textbf{long videos} is especially highly-demanded and emerging due to the flourishing growth of online videos in quantity and length.
% , and has become an essential task in multi-modal video understanding with its wide applications in video retrieval, video editing and video question answering.
% Video grounding is challenging since it relies heavily on the accurate understanding of textual query and video, as well as multi-modal alignment between them.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.99\linewidth]{Figures/intro_figure_3.pdf}
\end{center}
\caption{An example of long video temporal grounding, which requires coarse-to-fine multi-modal alignment.}
\label{fig:intro_figure}
\end{figure}

%fixed-length video \cite{lei2021detecting} or
%However, existing methods \cite{zhang2020span,zhang2020learning} mainly focus on datasets \cite{gao2017tall,krishna2017dense,lei2021detecting} with relatively short videos ranging from 0.5 to 2.5 minutes on average. 
However, limited by previously available datasets~\cite{gao2017tall,krishna2017dense,lei2021detecting}, existing works~\cite{zhang2020span,zhang2020learning} mainly deal with relatively short videos ranging from 0.5 to 2.5 minutes on average.
They typically downsample videos via uniform sampling to a fixed-length frame sequence. 


Recently, Ego4D~\cite{grauman2022ego4d} and MAD~\cite{soldan2022mad} datasets have been created and attempted to deal with long video, which spans from several minutes to three hours.
% Recent method for video grounding \cite{lei2021detecting} is built on Transformer-based architecture, which encodes the concatenated sequence of the entire video features and the feature of single text query using an unified encoder. 
\lj{two methods: down sample or sliding window}Directly applying existing methods to long video grounding poses two significant challenges:
(1) high inference computational cost  without reducing the sampling rate;
%when performing s on long videos
% entire long videos with variant lengths are hard to be modelled without decreasing the sampling rate, leading to high computational cost during inference;
(2) weaker matching ability to detailed contents due to the abundance of moment candidates.
% a large number of moment candidates from long videos makes their precise multi-modal alignment with the NL query more challenging.  
% the increased length of video contents will weaken the fine-grained alignment between each single video frame and the NL query. 
\lj{more clear} These issues result in information loss in both \textit{temporal aspect} (i.e., fewer visible frames with lower sampling rate) and \textit{contextual aspect} (i.e., weaker alignment to fine-grained contents like the objects, actions, scenes). 
\begin{comment}
weaker matching ability to the fine-grained content describing object and scene in video frames
\end{comment}
As the motivating example shown in Fig. \ref{fig:intro_figure}, accurate and reliable grounding requires a coarse-grained localization of relevant video segments (e.g. ``\textit{in the room}" v.s. ``\textit{outdoor}"), and fine-grained alignment to detailed object and action in frames (e.g., ``\textit{women}" and ``\textit{holding}").


To address these challenges, we propose \modelname, a window-centric coarse-to-fine alignment framework for long video temporal grounding.  
\lj{conclude before design details} The key advantage over prior works is that \modelname~simultaneously achieves outstanding performance and efficiency while keeping high frame sampling rate. 
% \modelname~flexibly handles long video inputs without decreasing the sampling rate, accelerates inference speed, and enhances coarse-to-fine multi-modal alignment for precise temporal grounding.
%  Firstly,slicing strategy and contrastive learning mechanism
To flexibly handle long videos, we slice the video into fixed-length candidate windows via a sliding window approach.
\lj{Centering at the windows, }we accelerate inference via coarse-grained (inter-window) pre-filtering, and enhance both coarse-grained and fine-grained (intra-window) multi-modal alignment with contrastive mechanisms.
% Centering at the sliding window, we propose to enhance training and inference via modelling coarse-grained (inter-window) to fine-grained (intra-window) alignment between videos and texts. 

%At coarse granularity, \modelname~accelerates inference speed for long videos.
%It utilizes a query-aware pre-filtering strategy to narrow down the sizable number of  windows that the model needs to consider by using a contrastive vision-text pre-trained model to compute semantic matching scores between the NL query and the candidate windows.

\lj{corase(window), joint (window+proposal), fine (proposal)}
At coarse granularity,  we accelerate inference speed via a query-aware pre-filtering strategy. It reduces the sizeable window number of the long video to a modest amount, based on their semantic matching score to the NL query computed by a contrastive vision-text pre-trained model~(e.g., CLIP).
%to compute semantic matching scores between the NL query and the candidate windows 
Furthermore, filtered video windows are semantically different and most are still irrelevant to the NL query. We then propose a window-based contrastive learning mechanism to model the semantic variance of inter-window pairs and further identify relevant windows. 
% Additionally, it helps the proposal generator to more accurately identify relevant windows in the video via a window-based contrastive learning mechanism. 
%This mechanism achieves this by 
Concretely, we select a contrasting negative window and design an inter-window contrastive loss during training.
% via the query-aware pre-filtering strategy of candidate windows.
% \modelname~also designs window-based contrastive learning mechanism to model the semantic variance of inter-window proposal pairs, and better identify relevant windows. 
% the window irrelevant to the text is hard to be identified by the model, which results in the unreliable ranking of inter-window proposals. 
% At coarse granularity, video windows are semantically different and are not necessarily relevant to the NL query.
% Therefore, modeling the inter-window semantic variance is important and is enhanced during training via a contrastive learning mechanism. 
% \modelname~also accelerates inference speed via the pre-filtering strategy of candidate windows.
% Therefore, we design window-based contrastive learning mechanism to capture the semantic differences of inter-window proposal pairs.
% Specifically, to accelerate inference when the number of candidate windows increased with longer video length, we present to pre-filter the candidate windows according to their semantic matching score to the NL query computed by the contrastive vision-text pre-trained model.
% Moreover, to help the proposal generator in identifying the relevant window, we conduct contrastive learning by selecting a contrastive negative window and designing inter-window contrastive loss to enhance training.  
%  by identifying their correspondence to the NL query. 
% Afterwards, to reduce the computational burden of the model during inference, we propose to pre-filter the candidate windows on the first stage by their semantic relevance to the NL query.
%such as scenes and objects

At fine granularity, reliable multi-modal alignment is demanding as the length of videos increases.
%aligning detailed contents  within intra-window moment proposals with NL queries becomes increasingly challenging as the length of videos increases.
To address this issue, we propose a fine-grained ranking strategy that utilizes a contrastive vision-text  pre-trained model (e.g., CLIP).  It computes fine-grained matching scores between each video frame and the NL query, which are further fused with proposal scores to reliably rank the intra-window moment proposals.
% the multi-modal alignment between the detailed content (e.g., scene and object) in intra-window moment proposals and the NL query is much more challenging when with increased length of videos.
% To solve this problem, \modelname~ incorporates a novel fine-grained ranking strategy, which utilizes the powerful multi-modal alignment ability of a large-scale contrastive pre-trained model (e.g., CLIP), to compute the fine-grained matching score of each video frame and the NL query. These scores are further fused to rank the intra-window moment proposals. 
% to enhance the multi-modal alignment between the fine-grained content (e.g., scene and object) of each single video frame and the NL query conditioned on video input with arbitrary length, \modelname~incorporates a novel ranking strategy for candidate proposals. 
% It utilizes the powerful multi-modal alignment ability of large-scale contrastive pre-trained model (e.g., CLIP), to compute the fine-grained matching score of each video frame and the NL query, which is further adopted to rank the candidate moment proposals. 

With the above design, \modelname~has the following advantages: (1) high efficiency and sampling rate on handling long video inputs (2) more accurate and reliable coarse-to-fine multi-modal alignment with less information loss.
%(1) flexibly handling long video inputs with high efficiency and sampling rate and (2) enhancing coarse-to-fine multi-modal alignment and alleviating information loss.
%~\zhijian{enhancing coarse-to-fine multi-modal alignment and providing optimal trade-off between performance and speed.}
% \begin{comment}
%\modelname~is evaluated on two large-scale long video grounding benchmarks. The state-of-the-art results and significant performance boosts (3.13\%$\rightarrow$6.87\% on MAD, and 10.46\%$\rightarrow$13.46\% on Ego4d-NLQ in terms of R1@IoU=0.3) on two datasets demonstrate the effectiveness of \modelname.
We evaluate \modelname~on two large-scale long video grounding benchmarks and achieve both the state-of-the-art results and significant performance boosts (3.13\%$\rightarrow$6.87\% on MAD, and 10.46\%$\rightarrow$13.46\% on Ego4D-NLQ in terms of R1@IoU=0.3).
%the effectiveness 
%The state-of-the-art results and significant performance boosts (3.13\%$\rightarrow$6.87\% on MAD, and 10.46\%$\rightarrow$13.46\% on Ego4d-NLQ in terms of R1@IoU=0.3) on two datasets demonstrate the effectiveness of \modelname.
% Extensive experiments demonstrate the effectiveness of the fine-grained ranking mechanism, and the flexibility of our method in processing video with different sampling rate and input length.
Further analysis shows that the pre-filtering
strategy shortens the inference speed by 2x for Ego4D-NLQ and 15x for MAD compared to inference on all candidate windows, without sacrificing its performance.
\begin{comment}
\zs{any justification we can provide, why such an approach cannot be used for ActivityNet etc.?}-\wanjun{Since we specifically focus on long video and the videos in these datasets are short, they are not suitable.}
\end{comment}
% \end{comment}
\paragraph{Contributions}
Our work presents two major contributions to the long video temporal grounding field. (1) We propose a novel coarse-to-fine alignment framework that utilizes a pipeline of \{slicing, pre-filtering, alignment\}, resulting in state-of-the-art performance and high efficiency on two representative benchmarks. 
%Our contributions are three-folded. 
%(1) We are one of the early works for long video temporal grounding, which can provide an effective baseline for future research.
(2) We introduce a novel approach for incorporating contrastive learning into multi-modal alignment. It exploits powerful contrastive vision-text pre-trained models and designs an inter-window contrastive mechanism. 
%(3) We propose a novel coarse-to-fine alignment framework that utilizes a pipeline of \{slicing, pre-filtering, alignment\}, resulting in state-of-the-art performance and high efficiency on two representative benchmarks. 
% (2) We enhance multi-modal alignment by introducing a novel contrastive learning mechanism, which concurrently exploits powerful contrastive text-vision pre-trained models and designs an inter-window contrastive mechanism.
% Our major contributions are listed as follows.
% (1) We propose a novel coarse-to-fine alignment framework for long video temporal grounding, which adopts \{slicing, pre-filtering, alignment\} pipeline to achieve SOTA performance and high efficiency on two benchmarks. 
% % (1) We propose a window-centric learning framework to support temporal grounding for long videos without decreasing the sampling rate.
% (2) We strengthen multi-modal alignment by introducing a novel contrastive learning mechanism in the proposal generator.
% strengthen coarse-to-fine multi-modal alignment via a coarse contrastive learning and fine-grained ranking.
% (3) Experiments demonstrate significant performance improvements on two long video grounding tasks, and exhibit higher efficiency in handling long video inputs. 

==> Paragraphs/1-Intro_depre.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.99\linewidth]{Figures/intro_figure_3.pdf}
\end{center}
\caption{An example of long video temporal grounding, which requires coarse-to-fine multi-modal alignment.}
\label{fig:intro_figure}
\end{figure}

\section{Introduction}
Video temporal grounding~\cite{anne2017localizing,gao2017tall} aims to localize temporal moments relevant to a given natural language~(NL) query from an untrimmed video, and has become an essential task in multi-modal video understanding with its wide applications in video retrieval, video editing and video question answering.
This task is challenging since it relies heavily on the accurate understanding of textual query and video, as well as multi-modal alignment between them.
\par
Moreover, temporal grounding for long videos is especially highly-demanded due to the flourishing growth of online videos in quantity and length.
%fixed-length video \cite{lei2021detecting} or
However, limited by previously available datasets~\cite{gao2017tall,krishna2017dense,lei2021detecting}, existing works~\cite{zhang2020span,zhang2020learning} mainly deal with relatively short videos ranging from 0.5 to 2.5 minutes on average. They typically downsample videos via uniform sampling to a fixed-length frame sequence. 
% Recent method for video grounding \cite{lei2021detecting} is built on Transformer-based architecture, which encodes the concatenated sequence of the entire video features and the feature of single text query using an unified encoder.
Thus, directly adopting existing methods for long video grounding raises several major challenges:
%(1) entire long videos with variant lengths are hard to be modelled without decreasing the sampling rate, leading to high computational cost and inference time ;
(1) lengthy video modeling is much harder without decreasing the sampling rate, and leads to high computational and inference costs;
%(1) long-form video modeling is much harder.  There is a natural tension between high sampling rate and fast inference speed.  
(2) enormous moment candidates from long videos make their precise multi-modal alignment with the NL query more arduous.  % the increased length of video contents will weaken the fine-grained alignment between each single video frame and the NL query. 
These issues result in information loss in both \textit{temporal aspect} (i.e., fewer visible frames caused by down-sampling) and \textit{contextual aspect} (i.e., weaker matching ability to the details in each frame, as it is perturbed by numerous frames). 
\begin{comment}
weaker matching ability to the fine-grained content describing object and scene in video frames
\end{comment}
As the motivating example shown in Fig. \ref{fig:intro_figure}, accurate grounding requires  a coarse-grained localization of relevant video segments from long videos (e.g. ``\textit{in the room}" v.s. ``\textit{outdoor}"), and fine-grained alignment to the contents in the frames (e.g., ``\textit{women}" and ``\textit{holding}").


To address the aforementioned challenges, we propose \modelname, a window-centric COarse-to-fiNE alignment framework for long video temporal grounding.  
The key advantage over prior works is that CONE simultaneously achieves outstanding performance and efficiency with high frame sampling rate.
%It flexibly handles long video inputs without decreasing the sampling rate, accelerates inference speed, and enhances coarse-to-fine multi-modal alignment for precise temporal grounding.
%  Firstly,slicing strategy and contrastive learning mechanism
To alleviate the high computational cost derived from high sampling rate,
we flexibly slice the long video into candidate windows via a sliding window approach, this reduces GPU computational cost per time within the window rather than the whole video. 
%to support long video inputs with variant lengths.
%We adopt the sliding window approach to slice the entire long video into several fixed-length candidate windows. 
%to enhance training and inference via modelling
%Centering on the sliding window, we further propose a  coarse-grained (inter-window) to fine-grained (intra-window) alignment between videos and texts. 

At coarse granularity, to remedy the high inference time increased with longer video length,  we exploit the contrastive pretrained text-vision models~(e.g., CLIP) to pre-filter the candidate windows according to their semantic matching score to the NL query. It significantly shortens the inference time and surprisingly keeps the satisfying performance. 
%perform the pre-filtering strategy. It
Furthermore, 
%the window irrelevant to the text is hard to be identified by the model, which results in the unreliable ranking of inter-window proposals. 
% At coarse granularity, 
filtered video windows are semantically different and are not necessarily relevant to the NL query.
%Therefore, modelling the inter-window semantic variance is important and is enhanced during training via another contrastive learning mechanism.
% Therefore, we design window-based contrastive learning mechanism to capture the semantic differences of inter-window proposal pairs.
%Specifically, to accelerate inference when the number of candidate windows increased with longer video length, we present to pre-filter the candidate windows according to their semantic matching score to the NL query computed by the contrastive vision-text pre-trained model.
%Moreover, 
We propose a contrastive learning mechanism to discriminate the window containing relevant information by selecting a contrastive negative window and designing inter-window contrastive loss to enhance training. 
%  by identifying their correspondence to the NL query. 
% Afterwards, to reduce the computational burden of the model during inference, we propose to pre-filter the candidate windows on the first stage by their semantic relevance to the NL query.

At fine granularity, 
%the multi-modal alignment between the detailed content (e.g., scene and object) in intra-window moment proposals and the NL query is much more challenging when the length of video features increases. To solve this problem, 
to mitigate the challenging multi-modal alignment issue between the detailed content (e.g., scene and object) and the NL query,
we incorporate a fine-grained ranking strategy and utilize the powerful multi-modal alignment ability of the contrastive pretrained text-vision for the second time. It computes the fine-grained matching score of each video frame and the NL query, and these scores are further fused to rank the intra-window moment proposals. 
% to enhance the multi-modal alignment between the fine-grained content (e.g., scene and object) of each single video frame and the NL query conditioned on video input with arbitrary length, \modelname~incorporates a novel ranking strategy for candidate proposals. 
% It utilizes the powerful multi-modal alignment ability of large-scale contrastive pre-trained model (e.g., CLIP), to compute the fine-grained matching score of each video frame and the NL query, which is further adopted to rank the candidate moment proposals. 

%%It flexibly handles long video inputs without decreasing the sampling rate, accelerates inference speed, and enhances coarse-to-fine multi-modal alignment for precise temporal grounding.

With the above design, \modelname~has the following advantages: (1) flexibly handling long video inputs with high efficiency and sampling rate and (2) enhancing coarse-to-fine multi-modal alignment and alleviating information loss.
%~\zhijian{enhancing coarse-to-fine multi-modal alignment and providing optimal trade-off between performance and speed.}
% \begin{comment}
\modelname~is evaluated on two benchmarks based on long videos. The state-of-the-art results and significant performance boosts (3.13\%$\rightarrow$6.87\% on MAD, and 10.46\%$\rightarrow$13.46\% on Ego4d-NLQ in terms of R1@IoU=0.3) on two datasets demonstrate the effectiveness of \modelname.
% Extensive experiments demonstrate the effectiveness of the fine-grained ranking mechanism, and the flexibility of our method in processing video with different sampling rate and input length.
Further analysis shows that the pre-filtering strategy increases the inference speed by 2x for Ego4d-NLQ and 15x for MAD compared to inference on all candidate windows without sacrificing its performance.
\begin{comment}
\zs{any justification we can provide, why such an approach cannot be used for ActivityNet etc.?}-\wanjun{Since we specifically focus on long video and the videos in these datasets are short, they are not suitable.}
\end{comment}
% \end{comment}
\paragraph{Contributions} Our contributions are threefold.
(1) We propose a novel coarse-to-fine alignment framework for long video temporal grounding. 
It  adopts \{slicing, pre-filtering, alignment\} pipeline to achieve both high sampling rate and fast inference speed.
%It simultaneously achieves three conditions: outstanding performance, fast efficiency, and high frame sampling rate. 
(2) We propose a novel incorporation of contrastive learning into multi-modal alignment. It concurrently exploits powerful contrastive text-vision pretrained models and designs an inter-window contrastive mechanism.
(3) Experiments demonstrate significant performance boosts and SOTA results on two long video grounding datasets. 
%(1) We propose a window-centric learning framework to% support temporal grounding for long videos without decreasing the sampling rate.
%(2) We strengthen coarse-to-fine multi-modal alignment via a coarse contrastive learning and fine-grained ranking.
%(3) Experiments demonstrate significant performance improvements on two long video grounding tasks, and exhibit higher efficiency in handling long video inputs. 

==> Paragraphs/1-Intro_new2.tex <==
\section{Introduction}
Video temporal grounding~\cite{anne2017localizing,gao2017tall} aims to locate specific moments in an untrimmed video relevant to a textual user query.
This is a crucial task in multi-modal video understanding, and can be applied to many practical applications such as video retrieval~\cite{xu2016msr}, video editing, and video question answering~\cite{lei2018tvqa,lei-etal-2020-tvqa}. 
% , and has become an essential task in multi-modal video understanding with its wide applications in video retrieval, video editing and video question answering.
% Video grounding is challenging since it relies heavily on the accurate understanding of textual query and video, as well as multi-modal alignment between them.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.99\linewidth]{Figures/intro_figure_3.pdf}
\end{center}
\caption{An example of long video temporal grounding, which requires coarse-to-fine multi-modal alignment.}
\label{fig:intro_figure}
\end{figure}

%fixed-length video \cite{lei2021detecting} or
%However, existing methods \cite{zhang2020span,zhang2020learning} mainly focus on datasets \cite{gao2017tall,krishna2017dense,lei2021detecting} with relatively short videos ranging from 0.5 to 2.5 minutes on average. 
Temporal grounding for \textbf{long videos} is especially highly-demanded and emerging due to the flourishing growth of online videos in quantity and length.
However, limited by previously available datasets~\cite{gao2017tall,krishna2017dense,lei2021detecting}, existing works~\cite{zhang2020span,zhang2020learning} mainly deal with relatively short videos ranging from 0.5 to 2.5 minutes on average. 
%They typically downsample videos via uniform sampling to a fixed-length frame sequence. 
Recently, Ego4D~\cite{grauman2022ego4d} and MAD~\cite{soldan2022mad} datasets have been created and attempted to deal with long video, which spans from several minutes to hours.

% Recent method for video grounding \cite{lei2021detecting} is built on Transformer-based architecture, which encodes the concatenated sequence of the entire video features and the feature of single text query using an unified encoder. 
%\lj{two methods: down sample or sliding window}
%Directly applying existing methods to 


%weaker matching ability
% a large number of moment candidates from long videos makes their precise multi-modal alignment with the NL query more challenging.  
% the increased length of video contents will weaken the fine-grained alignment between each single video frame and the NL query.
%\lj{players}
Early attempts for long video grounding extends existing VTG models %adopt either existing works 
for short videos through sparse sampling or a sliding window adaptation. %or its window-based adaptation. 
%\lj{del:Nevertheless, both attempts are not desirable. 
%to a fixed-length frame sequence
%} 
On the one hand, existing models for short videos typically downsample videos to a fixed-length frame sequence, which leads to \textit{temporal information loss} for long videos~(i.e., fewer visible frames via sparse sampling).
%Under the long video scenario, 
%and train the ground-truth window
%\lj{divide del:process}
%\lj{every del:the whole}
Besides, the window-based adaptation methods divide the long video into candidate windows and inference on  every candidate window, which leads to high inference computational cost.
%decreasing the sampling rate, which
%simple adaptation approaches only train the ground-truth window, but inference on the whole candidate windows,
%\lj{On the other hand, a large number of candidates from long videos makes their precise multi-modal alignment with the NL query more challenging. del:as the ground-truth frames are perturbed by abundant irrelevant frames, long video length undermines the fine-grained matching ability of current models,} 
On the other hand, massive moment candidates from long videos make their precise multi-modal alignment with the NL query more challenging,
which leads to \textit{contextual information loss}~(i.e., weaker alignment to fine-grained contents, i.e., objects, actions, and scenes). As the motivating example shown in Fig. \ref{fig:intro_figure}, accurate grounding requires a coarse-grained localization of relevant video segments (e.g. ``\textit{in the room}" v.s. ``\textit{outdoor}"), and fine-grained alignment to detailed object and action in frames (e.g., ``\textit{women}" and ``\textit{holding}").
%between each video frame and the textual query
%like the objects, actions, and scenes
%but inference on the whole candidate windows,
%do not punish negative windows during training
%deal with accurate multi-modal alignment
%via the window-based slicing and trains the ground-truth window via the existing models.   Furthermore, it is hard to , which leads to weaker matching ability to fine-grained contents like objects, actions, and scenes.
%it is hard to identify irrelevant windows and 
%because the model lacks contrastive loss to punish negative windows during training 
%As a result, it leads to \textit{temporal information loss} (i.e., fewer visible frames with lower sampling rate) and weak multi-modal alignment.
%These issues result in information loss in both \textit{temporal aspect} (i.e., fewer visible frames with lower sampling rate) and \textit{contextual aspect} (i.e., weaker alignment to fine-grained contents like the objects, actions, scenes). 
In conclusion, long video length poses two new challenges:
(1) higher inference computational cost due to the heavy  workload of input processing;
% without reducing the sampling rate
%when performing s on long videos
% entire long videos with variant lengths are hard to be modelled without decreasing the sampling rate, leading to high computational cost during inference;
(2) arduous multi-modal alignment due to the abundance of moment candidates.
\begin{comment}
weaker matching ability to the fine-grained content describing object and scene in video frames
\end{comment}


%for long video temporal grounding. 
%\lj{conclude before design details} The key advantage over prior works is that \modelname~simultaneously achieves outstanding performance and efficiency while keeping high frame sampling rate. 
% \modelname~flexibly handles long video inputs without decreasing the sampling rate, accelerates inference speed, and enhances coarse-to-fine multi-modal alignment for precise temporal grounding.
%  Firstly,slicing strategy and contrastive learning mechanism
%To flexibly handle long videos, we slice the video into fixed-length candidate windows via a sliding window approach.
%\lj{Centering at the windows, }we accelerate inference via coarse-grained (inter-window) pre-filtering, and enhance both coarse-grained and fine-grained (intra-window) multi-modal alignment with contrastive mechanisms.
% Centering at the sliding window, we propose to enhance training and inference via modelling coarse-grained (inter-window) to fine-grained (intra-window) alignment between videos and texts. 
%At coarse granularity, \modelname~accelerates inference speed for long videos.
%It utilizes a query-aware pre-filtering strategy to narrow down the sizable number of  windows that the model needs to consider by using a contrastive vision-text pre-trained model to compute semantic matching scores between the NL query and the candidate windows.
%\lj{corase(window), joint (window+proposal), fine (proposal)}
\zhijian{to do}\lj{add this paragraph, please check}
To address these challenges, 
we propose \modelname, a window-centric coarse-to-fine alignment framework that speeds up inference and enhances accurate multi-modal alignment for long videos. First, we slice the arbitrary long video into candidate windows. Then, CONE employs a query-guided window selection strategy for efficiency and introduces a coarse-to-fine mechanism for effectiveness.
%by a contrastive vision-text pre-trained model~(e.g., CLIP)
Specifically, the \emph{query-guided window selection} strategy reduces the candidate window number of the long video. Moreover, the \emph{coarse-to-fine} mechanism consists of three components to gradually align the multi-modal inputs via multi-scale granularity: 
%window matching, window-propose joint learning, and propose (fine granularity) reranking. 
(1) window (coarse granularity) matching to select the most relevant candidate windows; (2) window-proposal (coarse to fine granularity) joint learning to find out proposal candidates considering both inter-window and intra-window relations; (3) proposal (fine granularity) reranking to further select the perfect moment from candidate proposals. \lj{del:Notably, generating proposals from separate windows led the model to focus only on the positive windows with ground truth moment/proposal while neglecting plenty of negative windows during training. However, there are a large number of negative windows during inference. This results in the discrepancy between training and inference, thus it is essential to model the inter-window and intra-window relation simultaneously. Concretely, we select a contrasting negative window and design an inter-window
contrastive loss during training.}

At coarse granularity,  we accelerate inference speed via a query-aware pre-filtering strategy. It reduces the sizeable window number of the long video to a modest amount, based on their semantic matching score to the NL query computed by a contrastive vision-text pre-trained model~(e.g., CLIP).
%to compute semantic matching scores between the NL query and the candidate windows 
Furthermore, filtered video windows are semantically different and most are still irrelevant to the NL query. We then propose a window-based contrastive learning mechanism to model the semantic variance of inter-window pairs and further identify relevant windows. 
% Additionally, it helps the proposal generator to more accurately identify relevant windows in the video via a window-based contrastive learning mechanism. 
%This mechanism achieves this by 
Concretely, we select a contrasting negative window and design an inter-window contrastive loss during training.
%reliable multi-modal alignment is demanding as the length of videos increases.
%To address this issue,
At fine granularity, we propose a fine-grained ranking strategy that utilizes a contrastive vision-text  pre-trained model (e.g., CLIP). It computes fine-grained matching scores between each video frame and the NL query, which are further fused with proposal scores to rank the intra-window moment proposals reliably.


With this coarse-to-fine design, \modelname~has the following advantages: (1) high efficiency in handling long video inputs with less temporal information loss; (2) more accurate multi-modal alignment with less contextual information loss.
%(1) flexibly handling long video inputs with high efficiency and sampling rate and (2) enhancing coarse-to-fine multi-modal alignment and alleviating information loss.
%~\zhijian{enhancing coarse-to-fine multi-modal alignment and providing optimal trade-off between performance and speed.}
% \begin{comment}
%\modelname~is evaluated on two large-scale long video grounding benchmarks. The state-of-the-art results and significant performance boosts (3.13\%$\rightarrow$6.87\% on MAD, and 10.46\%$\rightarrow$13.46\% on Ego4d-NLQ in terms of R1@IoU=0.3) on two datasets demonstrate the effectiveness of \modelname.
We evaluate \modelname~on two large-scale long video grounding benchmarks and achieve both the state-of-the-art results and significant performance boosts (3.13\%$\rightarrow$6.87\% on MAD, and 10.46\%$\rightarrow$13.46\% on Ego4D-NLQ in terms of R1@IoU=0.3).
%the effectiveness 
%The state-of-the-art results and significant performance boosts (3.13\%$\rightarrow$6.87\% on MAD, and 10.46\%$\rightarrow$13.46\% on Ego4d-NLQ in terms of R1@IoU=0.3) on two datasets demonstrate the effectiveness of \modelname.
% Extensive experiments demonstrate the effectiveness of the fine-grained ranking mechanism, and the flexibility of our method in processing video with different sampling rate and input length.
Further analysis shows that the pre-filtering
strategy shortens the inference speed by 2x for Ego4D-NLQ and 15x for MAD compared to inference on all candidate windows, without sacrificing its performance.
\begin{comment}
\zs{any justification we can provide, why such an approach cannot be used for ActivityNet etc.?}-\wanjun{Since we specifically focus on long video and the videos in these datasets are short, they are not suitable.}
\end{comment}
% \end{comment}
\paragraph{Contributions}
Our work presents two major contributions to the long video temporal grounding field. (1) We propose a novel coarse-to-fine alignment framework that utilizes a pipeline of \{slicing, pre-filtering, alignment\}, resulting in state-of-the-art performance and high efficiency on two representative benchmarks. 
%Our contributions are three-folded. 
%(1) We are one of the early works for long video temporal grounding, which can provide an effective baseline for future research.
(2) We introduce a novel approach for incorporating contrastive learning into multi-modal alignment. It exploits powerful contrastive vision-text pre-trained models and designs an inter-window contrastive mechanism. 
%(3) We propose a novel coarse-to-fine alignment framework that utilizes a pipeline of \{slicing, pre-filtering, alignment\}, resulting in state-of-the-art performance and high efficiency on two representative benchmarks. 
% (2) We enhance multi-modal alignment by introducing a novel contrastive learning mechanism, which concurrently exploits powerful contrastive text-vision pre-trained models and designs an inter-window contrastive mechanism.
% Our major contributions are listed as follows.
% (1) We propose a novel coarse-to-fine alignment framework for long video temporal grounding, which adopts \{slicing, pre-filtering, alignment\} pipeline to achieve SOTA performance and high efficiency on two benchmarks. 
% % (1) We propose a window-centric learning framework to support temporal grounding for long videos without decreasing the sampling rate.
% (2) We strengthen multi-modal alignment by introducing a novel contrastive learning mechanism in the proposal generator.
% strengthen coarse-to-fine multi-modal alignment via a coarse contrastive learning and fine-grained ranking.
% (3) Experiments demonstrate significant performance improvements on two long video grounding tasks, and exhibit higher efficiency in handling long video inputs. 

==> Paragraphs/2-task-ori.tex <==

\section{Preliminaries}
\subsection{Task Definition}
\label{sec:task-definition}
Since never-ending video streams in real applications put higher demand on grounding on longer videos, in this paper, we will study the task of video temporal grounding (VTG) in a challenging setting with long video inputs. 
% In this paper, we study the task of video temporal grounding (VTG) in a challenging setting with long video inputs, because never-ending video streams in realistic applications put higher demand on grounding on longer videos.

Taking a natural language (NL) query $Q$ and a long video $V$ as the inputs, the task of VTG  requires the system to locate the matched moment $M$ from the video $V$ relevant to the query $Q$. Formally, video $V=[v_1, v_2, \dots, v_{L_{v}}]$ is a sequence of uniformly sampled video frames, and $L_{v}$ denotes the length of the sampled frames. 
The NL query $Q=[q_1, q_2,\dots, q_{L_q}]$ is a sequence of tokens with sentence length $L_q$. 
% starting with $[CLS]$ token. 
The moment $M$ is a sub-sequence of $V$ that relevant to $Q$.
% Given a natural language query \textbf{Q}, the problem of \lj{LVTG} is to locate matched moments \textbf{M} in an untrimmed and long-form video \textbf{V}. The textual query \textbf{Q} is composed of ${L_{q}}$ tokens, and we extract its token-level feature sequence \textbf{Q} = [$q_1$, $q_2$, ..., $q_{L_q}$] and sentence-level cls token feature \textbf{q} by the text branch of vision-text pre-trained model. 
% The video \textbf{V} is a sequence of image frames and can be uniformly decomposed into a sequence of non-overlapping
% snippets. \lj{Video snippet} is a very short clip which only contains
% a few frames for feature extraction. We similarly extract video visual feature sequence \textbf{V} = [$v_1,v_2,...,v_{L_{v}}$].
% A moment \textbf{M} is a subsequence of frames in a video \textbf{V}.
% \begin{comment}
% The query \textbf{Q} = [$q_1$, $q_2$, ..., $q_m$] is a textual query composed of $m$ tokens.
% We denote the untrimmed and lengthy videos as V = [$f_1,f_2,...,f_T$] and the language query as \textit{Q} = [$q_1,q_2,...,q_{L_{q}}$], where T and ${L_{q}}$ are the number of frames and words, respectively.
% \end{comment}
This task is challenging especially for long videos because 
the acceptable length $L_{v}$ of current models is limited, leading to the difficulties in processing the entire video. Moreover, the accurate multi-modal alignment between each $v_i$ and $Q$ is also harder when $L_{v}$ increases.
\subsection{Moment-DETR}
\label{sec:moment-detr}
To reliably generate candidate moment proposals for temporal grounding, we choose Moment-DETR~\cite{lei2021detecting} as the backbone of our framework because of its advanced performance and compact end-to-end framework. 
Moment-DETR is a Transformer-based method complied with encoder-decoder architecture. 

% %Besides competitive performances on several temporal grounding benchmarks, it can easily extend to multiple groundtruth moments setting.
% Compared to anchor-based 2D-Map pipeline~\cite{zhang2020learning}, it does not need to maintain a mass of proposals during prediction. Compared to proposal-free span-based pipeline~\cite{zhang2020span}, it has a decoder module, which simultaneously generates a few high-quality proposals to satisfy multiple ground-truth
% moments setting.
% We believe this design is more promising than  the 2D-Map or span-based counterparts.
%for short videos.
%Unlike two-stage propose-and-rank or one-stage star/end-timestamp-prediction pipelines,
Specifically, it takes the concatenated features of video frames and query tokens as the model input $\bm{X}=[\bm{V}; \bm{Q}]$, which is encoded by a Transformer-based encoder with outputs $E_{enc}\in \mathbb{R}^{(L_v+L_q)\times d}$. The Transformer-based decoder aims to generate moment proposal features $E_{dec}\in \mathbb{R}^{N\times d}$ with given $E_{enc}$ and a set of $N$ trainable moment queries (fixed number of trainable embeddings) as the inputs. Then, it has two prediction heads: (1) a \text{saliency prediction head} for frames, which computes \textbf{saliency scores} of frames $S(V,Q)\in \mathbb{R}^{L_v}$ through a linear layer; (2) a proposal prediction head, which uses one FFN layer and three FFN layers.
The first FFN layer is used to predict a two-class \textbf{proposal score} for moment proposal $i$: $(p_i,1-p_i)$ indicating whether it matches the ground truth, while the three FFN layers are to predict the moment center coordinate and the width of each proposal, which is further used to compute the start ($b_i$) and end ($e_i$) position of proposal $i$.

% Directly adopting 

% During training, it adopts Hungarian algorithm to perform the optimal bipartite matching between the groundtruths and predictions. 
% and three FFN layers to generate timestamp predictions $\{b_i, e_i\}$. $p_i$ is the foreground class probability as well as the proposal score, and $b_i, e_i$ are start and end timestamps for $i$-th  proposal.
% Video snippet and query token sequence representations are projected to the same dimension of size d via two-layer feed forward network~(FFN) and then concatenated at length dimension. The concatenated input features are then processed by an encoder-decoder architecture. The decoder input is a set of N trainable positional embeddings of size d, referred to as moment queries. For encoder output, it uses a FFN layer to predict saliency score sequence $S^{sal} \in \mathbb{R}^{L_{w}}$ for each video snippet. For decoder output, it uses one FFN layer to predict two-class foreground/background labels ($p_i,1-p_i$) and three FFN layers to generate timestamp predictions $\{b_i, e_i\}$. $p_i$ is the foreground class probability as well as the proposal score, and $b_i, e_i$ are start and end timestamps for $i$-th  proposal.
%\hat{y} = \{\hat{y_i}\}^{N}_{i=1}, 
% During training, it adopts Hungarian algorithm to perform the optimal bipartite matching between the groundtruths and predictions. 
%V = [f1; f2; : : : ; fT ]
%The video \textbf{V} is composed of ${L_{v}}$ non-overlapping clips, we similarly extract its visual feature sequence \textbf{V} = [$v_1,v_2,...,v_{L_{v}}$].
%where ${L_{v}}$ is visual feature number.
%We denote each visual feature covers the information of a low-length video clip, and
 %spanning one or multiple clips.

%To deal with long-form video,
% As uniform sampling for long-form video leads to information loss, we utilize the sliding window paradigm.
% We slide on the video feature sequence and split it into a sequence of $N_w$  fixed-length overlapped windows \textbf{V} = [$W_1,W_2,...,W_{N_w}$]. 
% Video window is composed of continuous $L_w$ visual feature, \textbf{$W_i$}=[$v_{wb_i+1},v_{wb_i+2},...,v_{wb_i+L_{w}}$], where  $wb_i$ is the feature start index. 
% We apply $int(L_{w}/2)$ as the window stride and add two relatively short windows \textbf{$W_1$}=[$v_1,v_2,...,v_{L_{w}/2}$] and \textbf{$W_{N_w}$}=[$v_{int(n/N_w)*N_w},...,v_n$] to ensure each timestamp is covered by exact two windows.
% We denote  positive window as the windows which have overlap with the ground-truth moment, and negative window as the remaining windows.  Note that the positive window may only have partial overlap with the ground-truth.



% \begin{comment}
% The query \textbf{Q} = [$q_1$, $q_2$, ..., $q_m$] is a textual query composed of $m$ tokens.
% We denote the untrimmed and lengthy videos as V = [$f_1,f_2,...,f_T$] and the language query as \textit{Q} = [$q_1,q_2,...,q_{L_{q}}$], where T and ${L_{q}}$ are the number of frames and words, respectively.
% \end{comment}
